M2N: Mesh Movement Networks for PDE Solvers

Mainstream numerical Partial Differential Equation (PDE) solvers require discretizing the physical domain using a mesh. Mesh movement methods aim to improve the accuracy of the numerical solution by increasing mesh resolution where the solution is not well-resolved, whilst reducing unnecessary resolution elsewhere. However, mesh movement methods, such as the Monge-Ampere method, require the solution of auxiliary equations, which can be extremely expensive especially when the mesh is adapted frequently. In this paper, we propose to our best knowledge the first learning-based end-to-end mesh movement framework for PDE solvers. Key requirements of learning-based mesh movement methods are alleviating mesh tangling, boundary consistency, and generalization to mesh with different resolutions. To achieve these goals, we introduce the neural spline model and the graph attention network (GAT) into our models respectively. While the Neural-Spline based model provides more flexibility for large deformation, the GAT based model can handle domains with more complicated shapes and is better at performing delicate local deformation. We validate our methods on stationary and time-dependent, linear and non-linear equations, as well as regularly and irregularly shaped domains. Compared to the traditional Monge-Ampere method, our approach can greatly accelerate the mesh adaptation process, whilst achieving comparable numerical error reduction.

==> command.tex <==
\usepackage{etoolbox}

%enable the next line to enable all color-coded comments
\newtoggle{color_coded_comments}
\toggletrue{color_coded_comments}
%\togglefalse{color_coded_comments}

\iftoggle{color_coded_comments}{
% enable color_coded_comments
\newcommand{\mingrui}[1]{\textcolor{blue}{Mingrui: #1}}
\newcommand{\wenbin}[1]{\textcolor{cyan}{Wenbin: #1}}

}
{
%disbable color_coded_comments
\newcommand{\mingrui}[1]{#1}
\newcommand{\wenbin}[1]{#1}
}
\newcommand{\zheng}[1]{{\bf \color{red} [Zheng: ``#1'']}}
\newcommand{\joe}[1]{{\bf \color{magenta} [Joe: ``#1'']}}
\newcommand{\xiang}[1]{{\bf \color{teal} [Xiang: ``#1'']}}
\newcommand{\fanglei}[1]{{\bf \color{brown} [Fanglei: ``#1'']}}

